Sim-Anchored Learning for On-the-Fly Adaptation

Fine-tuning simulation-trained RL agents with real-world data often degrades crucial behaviors due to limited or skewed data distributions. We argue that designer priorities exist not just in reward functions, but also in simulation design choices like task selection and state initialization. When adapting to real-world data, agents can experience catastrophic forgetting in important but underrepresented scenarios. We propose framing live-adaptation as a multi-objective optimization problem, where policy objectives must be satisfied both in simulation and reality. Our approach leverages critics from simulation as "anchors for design intent" (anchor critics). By jointly optimizing policies against both anchor critics and critics trained on real-world experience, our method enables adaptation while preserving prioritized behaviors from simulation. Evaluations demonstrate robust behavior retention in sim-to-sim benchmarks and a sim-to-real scenario with a racing quadrotor, allowing for power consumption reductions of up to 50% without control loss. We also contribute SwaNNFlight, an open-source firmware for enabling live adaptation on similar robotic platforms.

==> figs/sim-to-sim.tex <==
\centering
% Define colors
\definecolor{myblue}{HTML}{265285}
\definecolor{mypurple}{HTML}{8e0178}
\definecolor{mygreen}{HTML}{38aa38}
\definecolor{myorange}{HTML}{ee6e00}
\definecolor{myred}{HTML}{e41a1c}
\definecolor{mypink}{HTML}{984ea3}

\newlength{\barwidth}
\setlength{\barwidth}{7pt}
\newlength{\plotsep}

% Load the data
\pgfplotstableread[col sep=comma]{
env,method,A_value,A_error,B_value,B_error
Pendulum-v1,naive,-39.85,10.57,0.08,3.62
Pendulum-v1,ours,9.96,2.12,5.02,15.10
Reacher-v4,naive,-21.01,24.79,-0.96,7.42
Reacher-v4,ours,6.24,13.29,2.00,14.01
LunarLander-v2,naive,-41.07,33.22,0.72,26.87
LunarLander-v2,ours,-49.91,19.94,-5.18,21.27
}\datatable

% Common style for all plots
\pgfplotsset{
    common style/.style={
        width=0.14\textwidth,
        height=4cm,
        ybar,
        ymajorgrids=true,
        grid style=dashed,
        ymin=-70,
        ymax=70,
        ytick={-50,0,50},
        error bars/y dir=both,
        error bars/y explicit,
        enlarge x limits=1.0,
        xtick pos=bottom,
        yticklabel style={font=\scriptsize},
        symbolic x coords={A,B},
        xtick={A,B},
        x tick label style={font=\scriptsize},
    }
}

% Define a command for creating a single plot
\newcommand{\singleplot}[4]{
    \nextgroupplot[yticklabels={#2},]
    \pgfplotstablegetelem{#3}{A_value}\of\datatable
    \pgfmathsetmacro{\valueA}{\pgfplotsretval}
    \pgfplotstablegetelem{#3}{A_error}\of\datatable
    \pgfmathsetmacro{\errorA}{\pgfplotsretval}
    \pgfplotstablegetelem{#3}{B_value}\of\datatable
    \pgfmathsetmacro{\valueB}{\pgfplotsretval}
    \pgfplotstablegetelem{#3}{B_error}\of\datatable
    \pgfmathsetmacro{\errorB}{\pgfplotsretval}
    \pgfmathparse{\valueA < 0 ? "myred" : "mygreen"}
    \edef\tempcolorA{\pgfmathresult}
    \pgfmathparse{\valueB < 0 ? "myred" : "mygreen"}
    \edef\tempcolorB{\pgfmathresult}
    \addplot[
        fill=\tempcolorA,
        bar width=\barwidth,
        bar shift=0cm,
        error bars/.cd,
    ] coordinates {(A,\valueA) +- (0,\errorA)};
    \addplot[
        fill=\tempcolorB,
        bar width=\barwidth,
        bar shift=0cm,
        error bars/.cd,
    ] coordinates {(B,\valueB) +- (0,\errorB)};
    \node[anchor=north, font=\footnotesize] at (rel axis cs:0.5,1) {#4};
}

% Define a command for creating a pair of plots for one environment
\newcommand{\environmentplots}[4]{
    \begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=2 by 1,
            horizontal sep=0.01\textwidth,
        },
        common style,
    ]
    
    \singleplot{#1}{#2}{#3}{naive}
    \singleplot{#1}{,,}{#4}{ours}
    
    \end{groupplot}
    \node[above=0.1cm] at ($(group c1r1.north)!0.5!(group c2r1.north)$) {\textbf{#1}};
    \ifnum\pdfstrcmp{#1}{Pendulum-v1}=0
        \node[rotate=90, anchor=south, font=\small] at ($(group c1r1.west)!0.5!(group c2r1.west)-(1.2cm,0)$) {Reward Delta};
    \fi
    \end{tikzpicture}%
}

% Create the plots
\environmentplots{Pendulum-v1}{-50\%,0\%,+50\%}{0}{1}
\hfill
\environmentplots{Reacher-v4}{,,}{2}{3}
\hfill
\environmentplots{LunarLander-v2}{,,}{4}{5}

